The Adjacent Fragment and Quine's Limits of Decision

We introduce the adjacent fragment AF of first-order logic, obtained by restricting the sequences of variables occurring as arguments in atomic formulas. The adjacent fragment generalizes (after a routine renaming) the two-variable fragment of first-order logic as well as the so-called fluted fragment. We show that the adjacent fragment has the finite model property, and that the satisfiability problem for its k-variable sub-fragment is in (k-1)-NExpTime. Using known results on the fluted fragment, it follows that the satisfiability problem for the whole adjacent fragment is Tower-complete. We additionally consider the effect of the adjacency requirement on the well-known guarded fragment of first-order logic, whose satisfiability problem is TwoExpTime-complete. We show that the satisfiability problem for the intersection of the adjacent and guarded adjacent fragments remains TwoExpTime-hard. Finally, we show that any relaxation of the adjacency condition on the allowed order of variables in argument sequences yields a logic whose satisfiability and finite satisfiability problems are undecidable.

==> sections/guarded-fragment-old.tex <==
%!TEX root = ../adjFrag.tex

\section{The Guarded Subfragment}\label{sec:guarded}
\begin{center}
	\verb+<This section under construction>+
\end{center}

We next shift our attention to the \emph{guarded adjacent fragment}, 
denoted~$\GA$, defined as the intersection of $\AF$ with the well-known guarded fragment, $\GF$~\cite[Sec.~4.1]{ABN98}. 
%\bbe{of first-order logic by H.~Andr\'eka, J.~van~Benthem, and I.~N\'emeti}.
In $\GF$, quantification is relativized by atoms, e.g. all quantification 
takes the form $\forall{\bar{x}} (\alpha \rightarrow \psi)$ and $\exists{\bar{x}} (\alpha \land \psi)$, where $\alpha$ (a \emph{guard}) is an atom featuring all 
the variables in $\bar{x}$ and all the free variables~of~$\psi$. The satisfiability problem for $\GF$ is $\TwoExpTime$-complete, falling to 
$\ExpTime$-complete for its $k$-variable sub-fragment~\cite{Gradel99}.
We show that the satisfiability problem for $\GA$ remains $\TwoExpTime$-complete, and thus is as hard as for full $\GF$.


Our proof employs the same reduction strategy as the $\TwoExpTime$-hardness 
proof for $\GF$ by E.~Gr\"adel~\cite[Thm.~4.4]{Gradel99}.
%The novel part of the reduction here concerns a feature characteristic of 
%hardness results for guarded logics~\cite{Gradel99,Kieronski19}. 
Because we are working in the guarded \emph{adjacent} fragment, however, Gr\"adel's reduction is no longer available, and new techniques are required. 
To aid readability, we employ the variable names $w, x, y, z, \dots$ in adjacent formulas,  rather than the official $x_1, x_2, x_3, x_4, \dots$. The reader 
may easily check that all formulas in question are indeed in $\AF$ modulo variable renaming.

\subsection{Generating Words.}
We start with a combinatorial exercise concerning the generation of word sequences by the recurrent application of certain adjacent functions. 
Let $m \in \N$ and consider the adjacent functions $\lambda_1, \lambda_2, \lambda_1 \colon [1,m+2] \rightarrow [1,m+1]$ defined as follows 
(the upper index is mapped to the lower~one):
\begingroup % nasty hack
\setlength\arraycolsep{6pt}
\begin{align*}
    \lambda_{1} & \coloneqq 
        \begin{pmatrix}
        1 & 2 & 3 & 4 & 5 & \dots & m{+}2\\
        1 & 2 & 2 & 3 & 4 & \dots & m{+}1
        \end{pmatrix}, \;
    \lambda_{2} \coloneqq 
        \begin{pmatrix}
        1 & 2 & 3 & 4 & 5 & \dots & m{+}2\\
        1 & 2 & 1 & 2 & 3 & \dots & m
        \end{pmatrix},
    %
    % \lambda_{3} \coloneqq 
    %     \begin{pmatrix}
    %     1 & 2 & 3 & 4 & 5 & \dots & m{+}2 \\
    %     1 & 2 & 3 & 3 & 4 & \dots & m{+}1
    %     \end{pmatrix}.
\end{align*}
\endgroup
\begingroup % nasty hack
\setlength\arraycolsep{3pt}
\begin{align*}
    \lambda_{3} \coloneqq 
        \begin{pmatrix}
        1 & 2 & 3 & 4 & 5 & \dots & m{+}2 \\
        1 & 2 & 3 & 3 & 4 & \dots & m{+}1
        \end{pmatrix}.
\end{align*}
\endgroup
We show that repeated application of these functions to the bit-string $\bfz \bfo \bfo^m$ yields the whole of the language
$\bfz \bfo \{ \bfz, \bfo \}^m$.
%
\begin{lemma} \label{lemma_GA_generation_1}
    Let $W_0 \subseteq \{ \bfz, \bfo \}^*$ contain $\bfz \bfo \bfo^m$ and $W_i \coloneqq W_{i{-}1}$
    $\cup \{ \bar{w}^{\lambda_1}, \bar{w}^{\lambda_2}, \bar{w}^{\lambda_3} \mid \bar{w} \in W_{i{-}1} \}$.
    Setting $W \coloneqq \textstyle \bigcup_{i\geq0} W_i$, we have $\bfz \bfo \{ \bfz, \bfo \}^m \subseteq W$. %Then $\bfz \bfo \{ \bfz, \bfo \}^n \subseteq \textstyle \bigcup_{i\geq0} W_i$.
\end{lemma}   
\begin{proof}
We establish by induction on  $i$ ($0 \leq i \leq m$) that, for any word $\bar{c} \in \{ \bfz, \bfo \}^i$, 
the word $\bfz \bfo \bar{c} \bfo^{m{-}i}$ is in $W$; the case $i = m$ then yields the statement of the lemma.
The base case, $i = 0$ follows from the assumption that $W_0$ contains $\bfz\bfo\bfo^m$. Suppose now $i > 0$. 
We show that, for any $x\in \{ \bfz, \bfo \}$, the word $u = \bfz \bfo x \bar{c} \bfo^{m{-}i{-}1}$ is in $W$.
Letting $c_1$ be the first character of $\bar{c}$, and writing $\bar{c}= c_1\bar{d}$, it follows by 
inductive hypothesis that the words $\bar{v} = \bfz \bfo \bar{c}\bfo^{m{-}i{-}1} \bfo$ and
$\bar{w} = \bfz \bfo \bar{d} \bfo^{m{-}i{-}1} \bfo \bfo$ are in $W$.
We consider the following cases: 
(i) if $x = \bfo$ then $\bar{u} = \bar{v}^{\lambda_1}$, 
(ii) if both $x$ and $c_1 = \bfz$ then $\bar{u} = \bar{v}^{\lambda_3}$,
and otherwise, (iii) $x=\bfz$, $c_1 =  \bfo$ and $\bar{u} = \bar{w}^{\lambda_2}$.
Thus~$\bar{u} \in W$.
\end{proof} 

We now apply Lemma~\ref{lemma_GA_generation_1} to $\GA$.
Let $P$ be a binary predicate and $G_{m}$ an $(m{+}2)$-ary predicate ($m \geq 0$). 
%\bbe{(``the generator of size $m$'')}. 
We wish to write a sentence $\zeta^P_{m}$ of $\GA$ ensuring that, if $P$ is satisfied by a pair of objects $ab$, then
$G_{m}$ is satisfied by any $(m+2)$-tuple $ab\bar{a}$, where $\bar{a}$ is a word of length $m$ over the alphabet $\set{a, b}$.
It follows immediately from Lemma~\ref{lemma_GA_generation_1} that the following suffices:
\begin{multline*}
\zeta^P_{m} \coloneqq \forall x y \; \Big( P(x y) \to
        G_{m}(x y \underbrace{y \cdots y}_m) \Big) \land\\
    \bigwedge_{i \in [1,3]} \forall \bu_{m+2} \; 
        \Big( G_{m}(\bu_{m+2}) \to
        G_{m}(\bu_{m+2}^{\lambda_i}) \Big).
\end{multline*}
%
We shall require a `mirrored' version of the above device, this time involving a \textit{pair} of 2-element alphabets and a {\em pair} of
words of length $m$ over these alphabets. Let $R$ be a $4$-ary predicate 
%\bbe{(representing ``concatenated positions'')} 
and $F_m$ a $(2m + 4)$-ary predicate ($m \geq 0$).
%\bbe{(yet another but larger ``generator'' predicate)}. 
We wish to write a sentence $\epsilon^{R}_{m}$ of $\GA$ ensuring that, if $R$ is satisfied by a quartet of objects 
$baa'b'$, then, for any $m$-tuple $\bar{a}$ over the alphabet $\set{a, b}$, and any $m$-tuple $\bar{a}'$ over the alphabet $\set{a', b'}$,
the predicate $F_{m}$ 
is satisfied by $\bar{a}baa'b'\bar{a}'$.  We denote by $\lambda_0$ the identity function on $[1,m+2]$,
and we take $\lambda_1, \lambda_2, \lambda_3$ to be as above. In addition, we write $\tilde{\bu}_{m+2}$ for the
tuple of variables $z_{m+2} \cdots z_1$ and $\bv_{m+2}$ for the
tuple of variables $z'_1 \cdots z'_{m+2}$. It follows from two applications of Lemma~\ref{lemma_GA_generation_1} that the following 
definition of $\epsilon^{R}_{m}$ suffices:
\begin{multline*}
\epsilon^{R}_{m}\coloneqq
    \forall y x x' y' \; \Big( R(y x x' y') \to
        F_m(\underbrace{y \dots y}_m y x x' y' \underbrace{y' \dots y'}_m) \Big) \wedge \\
    \bigwedge_{i, j \in \{0,1,2,3\}} \hspace{-1.75em}\forall \tilde{\bu}_{m+2} \bv_{m+2} \; 
        \Big( F_m(\tilde{\bu}_{m{+}2} \bv_{m+2}) \to \\
        F_m(z_{\lambda_{i}(m+2)} \dots z_{\lambda_{i}(1)} z'_{\lambda_{j}(1)} \dots z'_{\lambda_{j}(m+2)}) \Big).
\end{multline*}

\subsection{ATMs.} We employ the standard device of~\emph{Alternating Turing Machines} (ATMs)~\cite{Chandra81}. 
\begin{center}
	The presentation of ATMs here was an utter mess. It needs completely re-doing.
\end{center}
%Any ATM may be specified as a tuple $\tm = \langle \tmst, \tmal, \tmtrl, \tmtrr, q_0, \kappa \rangle$, 
%where $\tmst$ is a finite set of \textit{states},
%$\tmal$ is a finite alphabet, 
%% containing an empty-cell symbol `$\blank$',
%$\tmtrl, \tmtrr\colon \tmst \times \tmal \to \tmst \times \tmal \times [-1, 1]$ are, 
%respectively, the \textit{left-} and \textit{right-transition relations},
%$q_0 \in Q$ is the \textit{initial state}, and
%$\kappa: \tmst \rightarrow \{ \tmuni, \tmexi \}$ is function specifying stating whether a given state is, respectively, 
%\emph{universal} $\tmuni$ or \emph{existential} $\tmexi$. 
%A {\em configuration} of $\tm$ is a tuple
%$\langle q,\bar{s},h\rangle$, where
%$q \in \tmst$ is a machine state, $\bar{s} \in \tmal^m$ \bbe{is} a word indicating the contents of the tape,
%and $h \in [0, m-1]$ \bbe{is} an integer indicating the position of the head at some point in the computation.
%The {\em initial configuration} with input $\bar{x}$ is 
%
%
%An ATM defines a tree of configurations, with the initial
%configuration at the root, and the daughters of any configuration generated by the left- and right-transition relations. 
%The set of {\em accepting} configurations in this computation is the smallest set satisfying the following conditions:
%A configuration 
%
%
%
%By tracking every step of the computation by $\tm$ on \bbe{a word} $\bar{w} \in \tmal^*$
%we obtain a binary tree structure $\tmct \coloneqq \langle \tmctver, \tmctverl, \tmctverr \rangle$ \bbe{(where, as usual, $\tmctver$ is the set of vertices of $\tmct$, while $\tmctverl$ and $\tmctverr$ are, respectively, the left child and the right child relations)}. 
%
%
%
%Each node $v \in \tmctver$ is labelled with some 
%
%
%
%
%
%Each edge $(v, u) \in \tmctvera$ \bbe{(for any $\eta \in \{ l,r \}$)} is labelled by a transition $\tmtra(q, s_h)$, enabled in the configuration~labelling~of~$v$.
%We call $\tmct$ the \emph{configuration tree} of the computation by $\tm$ on $\bar{w}$. 
%Assuming $\tmct$ is finite,
%we say that it is \emph{accepting} if no node is associated with a rejecting state.
%We identify the following three properties of $\tmct$.
%The root node is labelled with a configuration in which the machine is in state $q_0$, the head position is 
%$0$, and the tape is written with the string $\bar{w}$ followed by blanks.
%We call this property \emph{initial configuration} (\textbf{IC}).
%Let $u$ be a node labelled with a configuration in which the machine is in state $q$.
%If $q$ is universal, then $u$ will have two children; if $q$ is existential, then $u$ will have a single child; if $q$ is accepting, or rejecting then $u$ will have no children.
%
%
%
%We say that a state $q$ is  if 
%
%
% $\kappa(q) = \tmuni$, and there are no possible transitions given by $\tmtrl(q, s)$ and $\tmtrr(q, s)$ for any symbol $s \in \tmal$.
%\bbecomment{[There is something strange going on here. We define accepting states but we never use them with the exception of the sentence a few lines below regarding the total number of children.]}
%Dually, $q$ is \emph{rejecting} if and only if $\kappa(q) = \tmexi$, and, again, there are no possible transitions.
%%Given a word $\bar{\omega} \in \tmal^*$ we call $\tm(\bar{\omega})$ a \emph{run of $\tm$ on input $\bar{\omega}$}.
%
%\bbecomment{[This is contradictory. You define accepting states to be universal and then at the same time they should have 0 and 2 successors.]}
%We call this property \emph{successor existence}~(\textbf{SE}).
%Suppose further that, in the configuration labelling of some node~$u$ we have that the head is reading the symbol $s$ whilst in state $q$. Then any child~$v_\eta$ (such that $(u, v_\eta) \in \tmtra$, \bbe{where~$\eta$ is either $l$ or $r$}) represents the result of a single transition $\tmtra(q, s) = (p, s', k)$, and thus is labelled with a configuration \bbe{$p$} in which the machine state, \bbe{the symbol} $s'$ is written in place of $s$, and the head is moved by a distance of $k$.
%We call this property \textit{configuration succession}~(\textbf{CS}).

\subsection{Encoding numbers.} 
In the sequel, we will consider structures $\str{A}$ interpreting a unary predicate $O$. 
Whenever $\fA \models \alpha[ab]$, where $\alpha(xy)$ is the formula $\lnot O(x) \land O(y)$, we say that $a$ and $b$ \emph{act as zero and unit bits}, 
and for any word $\bar{c} \in \{a,b\}^+$, we write $\val{\fA}(\bar{c})$ to denote the integer represented by $\bar{c}$, considered as a bit-string, with $a$ 
standing for 0 and $b$ for 1
(most significant bit first).
Notice that there may be other elements, say $c$ and $d$, such that 
$\fA \models \alpha[cd]$, in which case may write $\val{\fA}(\bar{d})$ for the integer represented by any word $\bar{d} \in \{c,d\}^+$.
It is then straightforward to write a $\GA$-formula $\textsc{eq}(\bar{x} \bar{y})$ satisfying the property that
$\fA \models \textsc{eq}[\bar{c}\bar{d}]$ if and only if $\val{\fA}(\bar{c}) = \val{\fA}(\bar{d})$. For example, writing $\bu_m$ for $z_1 \cdots z_m$ and 
$\bv_m$ for $z'_1 \cdots z'_m$, we define: 
\begin{align*}
&
\shless{\bu_m}{\bv_m} \coloneqq \bigvee_{i=1}^m \Big( \neg O(z_i) \wedge O(z'_i) \wedge 
\bigwedge_{j = i + 1}^{m} \big( O(z_j) \leftrightarrow O(z'_j) \big) \Big).\\
\end{align*}
Similarly, one can write $\GA$-formulas satisfying the following properties:
\begin{itemize}\itemsep0em
	\item $\fA \models \shless{\bar{c}}{\bar{d}}$ iff $\val{\fA}(\bar{c}) < \val{\fA}(\bar{d})$ \label{GAF_less_def}
	\item $\fA \models \sheq{\bar{c}}{\bar{d}}$ iff $\val{\fA}(\bar{c}) = \val{\fA}(\bar{d})$
	\item $\fA \models \sheq{\bar{c}}{\bar{d}{+}k}$ iff $\val{\fA}(\bar{c}) = \val{\fA}(\bar{d}) + k$, for each $k \in \{ -1, 0, 1\}$.
\end{itemize}
The details are routine. We give, as an example, the formula 
%Given two bit-strings $\bar{c}$ and $\bar{d}$ (not necessarily composed of the same elements) there is a classical 
%way~\cite[p. ???]{PrattHartmann23} \bbecomment{[Ian, please fix.]} to define the following properties in the monadic fragment of $\FO$ (hence also in $\GA$ \bbe{with the proviso that the free variables are appropriately guarded}).
%
\begin{align*}
%    \sheq{\bu_m}{\bv_m} & \coloneqq & \bigwedge_{i = 1}^{m} \Big( O(z_i) \leftrightarrow O(z'_i) \Big),\\
%%
%    \sheq{\bu_m}{\bv_m + 0}  & \coloneqq & \sheq{\bu_m}{\bv_m},\\
%%
%    \sheq{\bu_m}{\bv_m - 1}  & \coloneqq & \sheq{\bv_m}{\bu_m +~1},\\
%
& \sheq{\bu_m}{\bv_m{+}1} \coloneqq \bigwedge_{i = 1}^{m} \Big( \big( O(z_i) \leftrightarrow O(z'_i) \big) \leftrightarrow \bigvee_{j=1}^{i-1} O(z_j) \Big).
\end{align*}

\subsection{The reduction.}
Fix an ATM $\tm$
working in space bounded by $2^{p(|\bar{w}|)}$ for a given input $\bar{w}$, with $p$ a polynomial.
Our goal is to construct, in space bounded by a logarithmic function of $|\bar{w}|$, 
a $\GA$-sentence $\varphi_{\tm, \bar{w}}$ 
satisfiable if and only if $\tm$ accepts $\bar{w}$.
By a standard padding argument, we may assume without loss of generality that $\tm$ in fact
works in space bounded by $2^{|\bar{w}|}$; utilising the fact that $\AExpSpace$ equals $\TwoExpTime$~\cite[Cor.~3.6]{Chandra81}, 
we obtain the desired bound on $\GA$.

Suppose that $\tm$ accepts $\bar{w}$, and consider the computation tree for this input; thus the root of this tree is an
accepting node. Now delete any non-accepting nodes along with their sub-trees, yielding a tree $\tmct \coloneqq (\tmctver, \tmctverl, \tmctverr)$, and let $n \coloneqq |\bar{w}|$.
We consider structures interpreting binary predicates $V, R, Q_q$ (for each {state} $q \in \tmst$), quaternary 
predicates $E_l, E_r$ and $n$-ary predicates $H, S_s$ (for each {tape symbol}~$s \in \tmal$).
We say that $\str{A}_0$ \emph{embeds $\tmct$} if there is $f\colon \tmctver \to A_0 \times A_0$ such that for all~$v \in \tmctver$, the following hold:
\begin{enumerate}[label=(\alph*)]\itemsep0em
    \item $\fA_0 \models V[f(v)]$, \label{GAF:list_model_A_first};
    \item $\fA_0 \models R[f(v)]$ if $v$ is the root node;
    \item $\fA_0 \models E_\eta[f(u)^{-1}, f(v)]$ if $(u, v) \in \tmctvera$, \bbe{for each $\eta \in \{ l, r \}$};
    \item $\fA_0 \models Q_q[f(v)]$ if the configuration $v$ is in state $q$;
    \item $\fA_0 \models S_s[\bin{n}{f(v)}(i)]$ if $v$'s $i$-th tape cell has symbol $s$; and 
    \item $\fA_0 \models H[\bin{n}{f(v)}(i)]$ if $v$'s head is located over the $i$-th tape square. \label{GAF:list_model_A_last}.
\end{enumerate}
%
It is easy to define a structure $\str{A}_0$ embedding $\tmct$:
the domain $A_0$ is composed of fresh symbols $0_v, 1_v$ for 
each node $v \in \tmctver$, and for which we set $f(v) = (0_v,1_v)$.
% (Notice that $0_v1_v$ is a word over $A_0$ of length 2.)
We then interpret the predicates $V, R, E, Q_q, S_s$ and $H$ as required 
by conditions \ref{GAF:list_model_A_first}--\ref{GAF:list_model_A_last}.
\bbe{Till the end of our reduction}, we construct a $\varphi_{\tm, \bar{w}}$ in $\GA$ such that: 
(i) $\str{A}_0$ can be expanded to a model $\str{A}$ of $\varphi_{\tm, \bar{w}}$ \bbe{(thus witnessing the satisfiability of $\varphi_{\tm, \bar{w}}$)};
and (ii) every model of $\varphi_{\tm, \bar{w}}$ embeds~$\tmct$.

The first conjunct of $\varphi_{\tm, \bar{w}}$ requires pairs $(a,b)$ satisfying the predicate $V$ to act as zero bits and unit bits,
indicated by the predicate $O$:
%
\[
    \varphi_1 \coloneqq \forall x y \; \Big( V(x y) \to \neg O(x) \land O(y) \Big).
\]
%
%Given a pair of elements $a, b \in A$ satisfying $\fA \models \neg O[a]$ 
%and $\fA \models O[b]$, we treat these elements, respectively, as turned-off 
%and turned-on bits of the binary encoding of integers. 
%Thus for any sequence $\bar{u} \in \{a,b\}^+$ we can associate the 
%integer value given by the canonical map $\val{\fA}$.

We now add $\zeta^V_n$ and $\zeta^V_{2n}$ to the main formula $\varphi_{\tm, \bar{w}}$ \bbe{ensuring the proper behaviour of the ``generating predicates''.}
Recall that the sentence $\zeta^V_m$ features an $(m+2)$-ary predicate $G_m$, and ensures that,
if $\fA \models V[a b]$, then $\fA \models G_m[a b \bar{c}]$ for all $c \in \{a, b\}^m$.
\bbe{The use of $G_{n}$ and $G_{2n}$ is crucial as such predicate will serve as dummy guards in the forthcoming formulas.}
By writing
%
\begin{align*}
\varphi_2 & \coloneqq &  \bigwedge_{p, q \in \tmst}^{p \neq q}
        \forall x y \Big( V(x y) 
        \to \big( \neg Q_{p}(x y) \lor \neg Q_{q}(x y) \big) \Big),\\
%
\varphi_3 & \coloneqq &
    \bigwedge_{s, s' \in \tmal}^{s \neq s'}
       \forall x y \bu_n \Big(
           G_n(x y \bu) {\to} \lnot \big( 
                S_s(\bu_n) {\land} S_{s'}(\bu_n) \big)
       \Big), \text{and} \\
 %
 \varphi_4 & \coloneqq &
    \forall xy\bu_n\bv_n \bigg(
        G_{2n}(x y \bu_n \bv_n) \to \Big( 
            \big( H(\bu_n) \land H(\bv_n) \big) \to \sheq{\bu_n}{\bv_n}
        \Big) \bigg)
\end{align*}

%
respectively, we ensure that every configuration is in at most one state at a time,
every tape square of a configuration has at most one symbol, and the read-write head of any configuration is pointing to a single square at a time.
Note that all of these formulas are guarded. 
However, the advertised behaviour of the guard predicates $G_n$ and $G_{2n}$ means,
in essence, that the guards have no semantic~effect.

We now secure the property (\textbf{IC}). To do so, let us first abbriviate 
\begin{align*}
    \mu_1 & \coloneqq & Q_{q_0}(x y) \land H(\bin{n}{x y}(0)) \land \bigwedge_{i = 1}^{|\bar{w}|} S_{w_i}(\bin{n}{x, y}(i{-}1)),\\
    \mu_2 & \coloneqq & \shless{\bin{n}{x, y}(|\bar{w}| {-} 1)}{\bu_n} \to S_{\blank}(\bu_n).
\end{align*}
With the following formula 
%
\[
    \varphi_5 \coloneqq \exists xy \Big( V(x y) \wedge R(x y) \Big) \wedge
    \forall xy \Big( R(x y) \to
    \big( \mu_1 \wedge \forall \bu_n (G_n(x y \bu_n) \to \mu_2) \big) \Big),
\]
%
we ensure \bbe{the existence of} a root configuration in which
the machine state is $q_0$, the head is scanning square \bbecomment{[Is it clear what the square is?]}`0', and the tape is written with the string $\bar{w}$ followed by the requisite number of blanks.

\bbe{In the forthcoming formulas, it will be handy to introduce abbreviations for disjuction of state predicates.}
Let $\text{K}_{\tmuni}$ be the formula $\textstyle \bigvee^{\kappa(q) {=} \tmuni}_{q \in \tmst} Q_q(xy)$, 
and define $\text{K}_{\tmexi}$ analogously.
Similarly, we define $\text{K}_{\tmrej}$ to be a disjunction of rejecting states.
Now, the formula 
\begin{align*}
    \varphi_6 \coloneqq \forall x y ( V(x y) \to \neg \text{K}_{\tmrej}(x y) ) 
\end{align*}
ensures that no configuration is labelled with a rejecting state.%\ianside{There's a weakness here. Some conjucnts enforce properties SE, IS or whatever. Others are just hanging around. This is uneven. Not sure if this can be fixed now}

\bbe{As our next step, we} encode the transitions of $\tm$, securing the property~(\textbf{SE}). %\bbeside{do we need to say anything about acc state?}\ianside{See earlier remarks about states with no successors}
Let 
$\psi_{\tmuni}$ abbreviate the formula $\textstyle\bigwedge_{\eta \in \{ l, r \}}\exists x' y' E_\eta(y x x' y')$, and
$\psi_{\tmexi}$ abbreviate the formula $\textstyle\bigvee_{\eta \in \{ l, r \}}\exists x' y' E_\eta(y x x' y')$, \bbe{which are responsible for ``creating successors''}
Writing
\[
\varphi_7 \coloneqq \bigwedge_{k \in \{\tmuni, \tmexi\}} \forall y x \bigg( V(x y) \to
\Big( \text{K}_{k}(x y) \to \psi_k \Big) \bigg).
\]
we ensure that, if $\fA \models V[a, b] {\land} \text{K}_{k}[a b]$, then $\fA$ contains 
pairs encoding the appropriate successor configurations \bbe{of the configuration represented by the pair~$(a,b)$}.
\bbecomment{[But what about accepting states? Do we need them at all?]}

We next ensure that the transitions have the expected effect on the configurations they connect, securing
the property (\textbf{CS}). \bbe{To keep our formulas guarded}, we
need a further ``generating'' predicate, $F_n$, to act as a dummy guard.
\bbe{We~achieve this by} adding $\epsilon^{E_\eta}_{n}$ to the main formula (for both \bbe{directions} $\eta \in \{l,r\}$).
\bbe{This secures that} $\fA \models$ $F_n[\bar{c} b a a' b' \bar{c}']$
for all $a, b, a', b'$ such that $\fA \models E_\eta[b a a' b']$ 
with $\bar{c} \in \{ a, b \}^n$, $\bar{c}' \in \{ a', b' \}^n$.
The \bbe{forthcoming} formula $\varphi_8$ then ensures that any pair of parent and successor configurations 
have identical tape contents (possibly) except for the position scanned by the head. Indeed:
\begin{multline*}
    \varphi_8 \coloneqq \forall \bu_n y x x' y' \bv_n \; 
         F_n(\bu_n y x x' y' \bv_n) \to \\
            \bigg( \Big( \neg H(\bu_n) \land \sheq{\bu_n}{\bv_n} \Big) \to 
                \Big( \bigwedge_{s \in \tmal} \big( S_s(\bu_n) \to S_s(\bv_n) \big) \Big) 
        \bigg).
\end{multline*}
\bbe{We next aim to encode the proper behaviour of transitions of $\tm$. For convinience, we abbriviate:}
\begin{align*}
    \chi & \coloneqq & Q_p(x' y') \land [\sheq{\bv_n}{\bu_n} \to S_{s'}(\bv_n)] \land [\sheq{\bv_n}{\bu_n + k} \to H(\bv_n)].
\end{align*}
\bbe{To encode the transition $\tau_\eta$ of $\tm$, we define the sequence $\xi_{\tau_\eta}$ as:}
%
\[
    \forall \bu_n y x x' y' \bv_n \; 
	G_{2n}(\bu_n y x x' y' \bv_n) {\to}
	    \Big( \big( E_\eta(y x x' y') \land  Q_q(x y) \land H(\bu_n) \land S_s(\bu_n) \big) {\to}
	    \chi \Big).
\]
%
Assuming the transition $\tau_\eta$ is of the form $(q, s) \mapsto (p, s', k)$, the formula $\xi_{\tau_\eta}$
states that, if in a certain configuration, the machine state is $q$ and the head is reading symbol $s$, 
then in the $\eta$-side successor configuration defined by $\tmtra$, the machine state will be
$p$, the symbol $s$ will have been replaced by $s'$, and  the head will have moved by $k$ \bbecomment{[steps?]}.
To encode all possible transitions, we write $\varphi_9$ to be:
\begin{align*}
    \varphi_9 \coloneqq \bigwedge_{\eta \in \{ l, r \}}\bigwedge_{\tau_\eta \in \tmtra} \xi_{\tau_\eta}.
\end{align*}

\bbe{This concludes the construction of the desired $\GA$-formula $\varphi_{\tm, \bar{w}}$.}

\subsection*{Correctness.}
\bbe{We next establish the correctness of our reduction, starting from the following direction.}

\begin{lemma}
The formula $\varphi_{\tm, \bar{w}}$ is satisfiable.
\end{lemma}
\begin{proof}
    \bbe{We already established the existence of} $\fA_0$ embedding some accepting $\tmct$ as described \bbe{by conditions} \ref{GAF:list_model_A_first}--\ref{GAF:list_model_A_last}.
    We expand $\fA_0$ to $\fA$ by setting $A = A_0$ with
    \begin{enumerate}
        \item $\fA \models \lnot O[a]$ and $\fA \models O[b]$ if $\fA_0 \models V[ab]$,
        \item $\fA \models G_m[a b \bar{c}]$ where $\fA_0 \models V[a b]$ and $\bar{c} \in \{ a, b \}^m$ (for each $m \in \{n, 2n\}$),
        \item $\fA \models F_n[\bar{c} b a a' b' \bar{c}']$ where $\fA_0 \models S_\eta[b a a' b']$, $\bar{c} \in \{ a, b \}^n$ and
        $\bar{c}' \in \{ a', b' \}^n$ (where $\eta \in \{l,r\}$).
    \end{enumerate}
    Recalling that $\tmct$ contains an initial configuration (\textbf{IC}), we have that $\fA \models \varphi_5$.
    Additionally, \bbe{as} $\tmct$ {has the property} (\textbf{SE}), we see that $\fA \models \varphi_7$.
    Lastly, since $\tmct$ has the property (\textbf{CS}), we have that $\fA \models \varphi_8$.
    \bbe{Hence, it follows that} $\fA \models \varphi_{\tm, \bar{w}}$.
\end{proof}

We next establish the other direction of the proof.

\begin{lemma}
If $\fA \models \varphi_{\tm, \bar{w}}$ then $\tm$ accepts $\bar{w}$.
\end{lemma}
\begin{proof}
Suppose $\fA \models \varphi_{\tm, \bar{w}}$.
We construct an embedding $f\colon \tmctver {\to} A \times A$ for an accepting $\tmct$ by well-founded induction.
The following observations will be used. Suppose \bbe{that} $\fA \models V[ab]$. Intuitively, we think of the pair
$(a,b)$ as a node of the computation tree labelled by some configuration, as determined by the \bbe{family of} predicates $Q_q$, $S_s$ and $H$.
By $\varphi_2$, there is a unique \bbe{$q \in \tmst$ for which} $Q_q$ satisfied by $ab$.
Moreover, by $\varphi_3$, any bit-string $\bar{c} \in \{a, b\}^n$ satisfies a unique $S_s$ (for $s \in \tmal$).
Similarly, by $\varphi_4$, there is a unique bit-string $\bar{c} \in \{a, b\}^n$ satisfying $H$.

\bbe{For the base case of the induction, }
% Proceeding with the induction,
% for the base case, 
we pick $a, b$ such that $\fA \models R[ab]$.
By \bbe{the satisfaction of} $\varphi_5$ we see that $\fA \models Q_{q_0}[ab]$, $\fA \models H[\bin{n}{a, b}(0)]$, and $\fA \models S_{w_i}[\bar{c}]$ for each index $1 \leq i \leq |\bar{w}|$
with $\val{\fA}(\bar{c}) = i{-}1$  and $\fA \models S_{\blank}[\bar{c}]$ otherwise. \bbecomment{[There is something wrong here. $\bar{c}$ is undefined.]}
We then set $\tmctver \coloneqq \{ v \}$ and $f(v) \coloneqq ab$. Labeling $v$ with the state, tape and head position as suggested by \bbe{Conditions}
\ref{GAF:list_model_A_first}--\ref{GAF:list_model_A_last}, we 
have secured the property (\textbf{IC}).

For the inductive step, let $u$ be node which has been \bbe{recently} added to the tree.
Assume $u$ is labelled with a configuration in which the machine state $q$ is universal, and the head is at position $h$, reading symbol $s$.
If $q$ is accepting, then we stop.\bbecomment{[There is a problem here, as our formulas enforce that universal (so thus accepting) states always have successors. What do we do with them?]}  Otherwise, $\varphi_7$ guarantees that there are pairs $(a_\eta, b_\eta) \in A^2$
such that $\fA \models S_\eta[f(u)^{-1} a_\eta b_\eta]$ for both directions $\eta \in \{ l, r \}$.
Notice that by \bbe{the satisfiaction of} $\varphi_8$ if the configuration labelling $u$ has the symbol $s'$ written on $i$-th tape square  (for $i \neq h$), then $\fA \models S_{s'}[\bin{n}{a_\eta b_\eta}(i)]$.
Due to $\fA \models \varphi_9$ the pair $a_\eta b_\eta$ satisfies the predicate $Q_p$ that is in accordance with the transition $\tmtra(q, s)=(p, s', k)$.
Additionally, $\fA \models S_{s'}[\bin{n}{a_\eta b_\eta}(h)]$ and $\fA \models H[\bin{n}{a_\eta b_\eta}(h + k)]$.
%
We thus set $\tmctver \coloneqq \tmctver \cup \{ v_\eta \}$, $f(v_\eta) \coloneqq (a_\eta, b_\eta)$ and $\tmctvera \coloneqq \tmctvera \cup \{ (u, v_\eta) \}$ thus securing (\textbf{SE}).
By interpreting the state, tape and head position of $v_\eta$ as \bbe{indicated} by \bbe{Conditions} \ref{GAF:list_model_A_first}--\ref{GAF:list_model_A_last}
we see that $v_\eta$ is a proper successor of $u$ as required by (\textbf{CS}).
% The case for when $q$ is existential is similar.
\bbe{The case of existential $q$ is treated in total analogy.}
Since there are no rejecting states in configuration tree (\bbe{due to the satisfiaction} $\varphi_6$),
there is an initial configuration by (\textbf{IC}),
each parent has children complying with (\textbf{SE}),
and each parent-child pair conforms to (\textbf{CS}), we conclude that $\tmct$ is an accepting configuration tree.
\end{proof}

\bbecomment{[Note that in our construction, it could be that our computation tree is ``looping''. Is this ok for the reduction? If so, we need to provide a proper reference.]}

By applying the above lemmas, we conclude correctness of our reduction. We have thus proved:
\begin{theorem}
    The finite and unrestricted satisfiability problem for (equality-free) guarded adjacent fragment of first-order logic is $\TwoExpTime$-hard. 
\label{theo:hard}
\end{theorem}


==> sections/interpolation.tex <==
%!TEX root = ../main.tex

\subsection{Interpolation in Guarded Adjacent Fragment}

We turn finally to the study of basic 
model-theoretic properties of~$\GA$, specifically to expressivity and interpolation.
Say that a logic $\logicL$ has the \textit{Craig Interpolation Property}~(CIP) if,
for all $\logicL$-formulas $\varphi_0, \varphi_1$ (potentially with free variables)
satisfying $\varphi_0 \models \varphi_1$ there exists 
an $\logicL$-formula $\chi$ (an $\logicL$-\emph{interpolant})
that employs only predicates common to $\varphi_0$ and~$\varphi_1$,
such that $\varphi_0 \models \chi$ and~$\chi \models \varphi_1$.
The CIP for a 
logic does not imply the CIP for either weaker or stronger logics; for example, both $\FO$ and $\GF^2$~\cite{HooglandMO99} have the CIP, 
while $\GF$~does~not~\cite{HooglandMO99}.
Our main result is that $\GA$ has the CIP.\@
We note however that $\AF$ lacks the CIP.\@ 
This follows from Lemma~\ref{lemma:fo2-and-af-over-binary-sig-are-the-same}
and the fact that $\FOt$ lacks the CIP~\cite{MarxA98}.

We present additional definitions required for the proof, starting 
from a suitable notion of bisimulation~\cite{BednarczykJ22,gradel2014freedoms} for~$\GA$.
If $\bar{a}$ is an $m$-tuple from some set, we speak of a {\em walk} on $\bar{a}$ to mean either
a function $f \in \bA^m_k$ for some $k$ or the image $\bar{a}^f$, as the context demands.
Fix some signature~$\sigma$. 
A tuple $\bar{a}$ in $\str{A}$ is \emph{$\sigma$-live} if there 
is a predicate $R \in \sigma$ for which $\bar{a} \in R^{\str{A}}$, and
$\sigma$-alive (adjacent live) if at least one of its surjective walks~is~$\sigma$-live.
A non-empty subset~$\bisimZ$ of 
  $\textstyle\bigcup_{n=0}^{\infty} (A^n \times B^n)$
  is called a \emph{$\sigma$-bisimulation} between 
  a pair of pointed structures 
  $(\str{A},\bar{a})$ and~$(\str{B},\bar{b})$, if %and only if 
  $(\bar{a}, \bar{b}) \in \bisimZ$ and, for 
  all~$(\bar{c}, \bar{d}) \in \bisimZ$:

  \begin{description} \itemsep0em
    \item[\desclabel{(atomic harmony)}{bisim:atomic-harmony}] $\atp^\fA_{\sigma}[\bar{c}] = \atp^\fA_{\sigma}[\bar{d}]$ and both $\bar{c}$ and $\bar{d}$ are $\sigma$-alive;
    %
    \item[\desclabel{(forth)}{bisim:forth}] for any  \bbe{infix $\bar{c}_i\ldots\bar{c}_j$ of $\bar{c}$} and a 
  tuple $\bar{u}$ in $\str{A}$ with \bbe{$\bar{c}_i\ldots\bar{c}_j\bar{u}$} $\sigma$-alive, 
  there is a corresponding tuple $\bar{v}$ in $\str{B}$ making \bbe{$\bar{d}_i\ldots\bar{d}_j\bar{v}$}
  $\sigma$-alive and \bbe{$(\bar{c}_i\ldots\bar{c}_j\bar{u},\ \bar{d}_i\ldots\bar{d}_j\bar{v}) \in \bisimZ$};
    %
    \item[\desclabel{(back)}{bisim:back}] for any \bbe{infix $\bar{d}_i\ldots\bar{d}_j$ of $\bar{d}$} and a tuple $\bar{v}$ in $\str{B}$ 
  with \bbe{$\bar{d}_i\ldots\bar{d}_j\bar{v}$} $\sigma$-alive,~there is a corresponding tuple $\bar{u}$ in $\str{A}$ 
  making \bbe{$\bar{c}_i\ldots\bar{c}_j\bar{u}$} $\sigma$-alive and \bbe{$(\bar{c}_i\ldots\bar{c}_j\bar{u},\ \bar{d}_i\ldots\bar{d}_j\bar{v}) \in \bisimZ$}.
  \end{description}

\noindent
Let $\bar{a}$ and $\bar{b}$ be $n$-tuples from $\str{A}$ and $\str{B}$.
Pointed structures $\str{A}, \bar{a}$ and $\str{B}, \bar{b}$ are $\sigma$-bisimilar 
(denoted: $\str{A}, \bar{a} \bisimto_\sigma \str{B}, \bar{b}$)
if there is a $\sigma$-bisimulation between them. 
We also write $\bar{a} \bisimto_\sigma \bar{b}$, if $\str{A}$ and $\str{B}$ can be deduced from the context.
We write $\str{A}, \bar{a} \equiv_\sigma \str{B}, \bar{b}$ to indicate that 
for all $\GA$-formulas~$\varphi$ over the signature $\sigma$
we have $\str{A} \models \varphi[\bar{a}]$ if and only if 
$\str{B} \models \varphi[\bar{b}]$.
A first-order formula~$\varphi$ is called \emph{$\GA$-invariant}
if
$\str{A},\bar{a} \bisimto_{\sig(\varphi)} \str{B}, \bar{b}$ implies 
$\str{A} \models \varphi[\bar{a}] \Leftrightarrow \str{B} \models \varphi[\bar{b}]$,
i.e.~if pointed structures that are $\sig(\phi)$-bisimilar agree on $\phi$.
By adapting textbook proofs we get: 

\begin{theorem}\label{thm:linking-bisimilarity-and-equivalence}
  $\str{A}, \bar{a} \bisimto_{\sigma} \str{B}, \bar{b}$ 
  implies $\str{A}, \bar{a} \equiv_{\sigma} \str{B}, \bar{b}$.
  The converse holds over $\omega$-saturated $\str{A}$ and $\str{B}$.
  Moreover, every $\GA$-invariant first-order formula is equivalent to some $\GA$-formula.
\end{theorem}

We say that $\GA$-formulas $\varphi_0$ and~$\varphi_1$ are 
\emph{jointly consistent} 
if there exist $(\sig(\varphi_0)\cap\sig(\varphi_1))$-bisimilar pointed 
models $(\str{A}_0, \bar{a}_0) \models \varphi_0$ and 
$(\str{A}_1, \bar{a}_1) \models \varphi_1$.
Given such formulas, we can compute jointly consistent 
conservative extensions
$\textsf{nf}(\varphi_i)$ of $\varphi_i$ in~\emph{normal~form}:
\begin{align*}
\textsf{nf}(\varphi_i) \coloneqq H(\bar{x}) \land
\textstyle\bigwedge_j \forall{\bx_{\ell_j}} \Big( R_j^{i}(\bx_{\ell_j}) \to
\mathsf{Q}_j \bx_{\ell_j{+}1; \ell_j {+} k_j}\; 
S_j^{i}(\bx_{\ell_j {+} k_j}) 
\oplus_j \psi_j^{i} \Big),
\end{align*}
where the $H, R_j^i$ and $S_j^i$ are predicates, 
the $\psi_j^{i}$ quantifier-free $\GA$-formulas, 
the  $\mathsf{Q}_j$ are quantifiers ($\forall$ or $\exists$), 
and the $\oplus_j$ are the corresponding 
Boolean connectives ($\to$~or~$\land$).
The predicate $H$ is called the \emph{head}~of~$\textsf{nf}(\varphi_i)$
(we stress that heads of $\textsf{nf}(\varphi_0)$ and $\textsf{nf}(\varphi_1)$ are equal).
Subformulas of $\textsf{nf}(\varphi_i)$ conforming to the pattern 
$S(\bar{x}) \to \mathsf{Q}\bar{y}\ R(\bar{x}\bar{y}) \oplus \psi$ 
are referred to as the \emph{existential} or \emph{universal} 
\emph{requirements of}~$\textsf{nf}(\varphi_i)$ according 
as $\mathsf{Q}=\exists$ or $\mathsf{Q}=\forall$.

When reasoning about structures definable in $\GA$, one can confine 
attention to certain forest-like structures.
We employ the standard set-theoretic reconstruction of the notion of a (countable)
\emph{tree} as a prefix-closed subset of $\N^*$. 
We say that a structure $\str{T}$ is a $\sigma$-\emph{adjacent tree structure} ($\sigma$-ATS) 
if $T$ is a tree and for any $(\ell{+}1)$-ary predicate~$R \in \sigma$, $\bar{d} \in R^{\str{T}}$ implies 
that there is a node $\bar{w} \in T$ and natural numbers 
$n_1, n_2, \ldots, n_\ell$ 
such that $\bar{d}$ is a surjective walk on 
$\bar{e} \coloneqq (\bar{w}, \bar{w} n_1, \bar{w} n_1 n_2, \ldots, \bar{w} n_1 \ldots n_\ell)$. 
We call such $\bar{e}$ \emph{the core} of~$\bar{d}$ and denote it by~$\core(\bar{d})$.
(Note that every $\sigma$-live tuple in $\str{T}$ has a unique core.)
Note that nodes in $\str{T}$ are naturally ordered by $ <_{\textit{lex}}$, 
i.e. the lexicographic ordering on $\N^*$.
This ordering can be lifted to the lexicographic ordering $\preceq$ on cores 
of $\sigma$-live tuples, which intuitively traverses trees top-down.
It can be shown that $\preceq$ has the property  
$(\heartsuit){:}$ if $\bar{c} \prec \bar{d}$ have common elements 
then some non-empty infix of $\bar{c}$ is a prefix of $\bar{d}$.
A~$\sigma$-\emph{adjacent forest structure} ($\sigma$-AFS) is a domain-disjoint union of $\sigma$-ATSs.

By employing a suitable notion of unravellings, 
one can show that if normal form $\varphi_0$ and~$\varphi_1$ of $\GA$ are jointly consistent, 
then they have $(\sig(\varphi_0) \cap \sig(\varphi_1))$-bisimilar pointed 
AFS models $(\str{A}_i, \bar{a}_i) \models \varphi_i$  satisfying $\bar{a}_i \in H^{\str{A}_i}$.
By linking classical model-theoretic proofs with the aforementioned observations about normal forms and AFSs, we conclude:

\begin{lemma}\label{lemma:super-lemma-about-CIP}
  If, for any normal form $\GA$-formulas $\varphi_0$ and~$\varphi_1$ having 
  $(\sig(\varphi_0) \cap \sig(\varphi_1))$-bisimilar pointed AFS models 
  there exists a model of $\varphi_0 \land \varphi_1$, then $\GA$ has the~CIP.\@ 
\end{lemma}

\noindent Fix until the end of the section $\varphi_0$ and $\varphi_1$ 
as in the antecedent of~\cref{lemma:super-lemma-about-CIP}, 
and their $(\sig(\varphi_0) \cap \sig(\varphi_1))$-bisimilar pointed AFS models 
$(\str{A}_0, \bar{a}_0)$ and $(\str{A}_1, \bar{a}_1)$.
For brevity, let $\sigma_i \coloneqq \sig(\varphi_i)$ for $i \in [0,1]$, 
and let $\tau$ and $\sigma$ denote, respectively, 
the union and the intersection~of~$\sigma_i$.

To show that $\GA$ has the CIP, it suffices 
to produce a model of $\varphi_0 \land \varphi_1$.
Following~\cite{BednarczykJ22}, we will inductively construct a growing 
sequence of $\tau$-AFSs $\str{U}_0, \str{U}_1, \ldots$, 
whose limit $\str{U}$ is going to be the desired model of $\varphi_0 \land \varphi_1$. 
We start from $\str{U}_0 \coloneqq \str{A}_0 \cup \str{A}_1$.
Then, we traverse the resulting AFS in a top-down manner (formalized by $\preceq$), 
dealing with cores of maximal $\sigma$-alive tuples as they are encountered.
Consider now a core tuple $\bar{d}$ encountered in this traversal,
and 
suppose that some (not necessarily surjective) walk $\bar{e}$ on $\bar{d}$ 
is $\tau$-live. (Remember: $\tau= \sigma_1 \cup \sigma_2$.)
It may be that $\bar{e}$ violates
either some universal or some 
existential requirements of $\varphi_0 \land \varphi_1$. 
%
We call such a $\bar{d}$ \emph{broken}.
During the inductive step, we ``repair'' the broken tuples.
This is achieved by replacing the substructure 
rooted at $\bar{d}$  by copies of
subtrees of~$\str{A}_i$ rooted at previously traversed tuples that are bisimilar to $\bar{d}$. 
(Bisimilarity helps us
``complete'' $\sigma_i$-types to $\tau$-types in a coherent way.)
Unfortunately, this repair may introduce fresh broken tuples, 
which we need to handle during the next step of the induction.

Call a tuple $\bar{d}$ 
(i) \emph{$n$-fresh} if it belongs to $\str{U}_n$ but not to $\str{U}_{n{-}1}$, and $n$-\textit{aged} otherwise;
(ii) \emph{maximal}, if $\bar{d}$ is not a proper infix of some $\sigma$-alive tuple;
(iii) \emph{core}, if the core of $\bar{d}$ is $\bar{d}$ itself; 
and (iv) \emph{$\sigma$-segment} if $\bar{d}$ is maximal, $\sigma$-alive and core.
%When constructing $\str{U}$, 
We shall always define $\str{U}_n$ in such a way that, 
for every $n$-aged $\sigma_i$-alive tuple in $\str{U}_n$ there 
exists a tuple in $\str{A}_i$ with the same $\sigma_i$-adjacent type.
This is achieved by means of partial 
\emph{origin functions} $\ori_i : U^* \to (A_i)^*$ that, 
intuitively, map copies of elements to their originals in $\str{A}_i$.
For soundness of the construction, several technical criteria are 
imposed on $\ori_i$ for all $i \in [0,1]$. 
%
\begin{enumerate}[label=(\alph*)]\itemsep0em
%
\item For any $n$-aged $\sigma_i$-alive $\bar{u}$ in $\str{U}_n$, 
the value $\bar{v}_i \coloneqq \ori_i(\bar{u})$ is defined, and $\atp^{\str{U}_n}_{\sigma_i}[\bar{u}]$ 
is equal to $\atp^{\str{A}_i}_{\sigma_i}[\bar{v}_i]$
and for all adjacent maps $f$ 
we have $\ori_i(\bar{u}^f) = (\bar{v}_i)^f$.
Moreover, in case $\bar{u}$ is $\sigma$-alive, we additionally have
$\atp^{\str{U}_n}_{\tau}[\bar{u}] = \textstyle \bigcup_{i=0}^{1} \atp^{\str{A}_i}_{\sigma_i}[\ori_i(\bar{v}_i)]$
and $\ori_i(\bar{v}_0) \bisimto_\sigma \ori_i(\bar{v}_1)$. 

\item For any existential requirement 
$R( \bar{x} ) \to \exists \bar{y}\ S(\bar{x}\bar{y}) \land \psi$ 
of~$\varphi_i$ and any $n$-aged tuple $\bar{u}$ in~$R^{\str{U}_n}$,
there exists a tuple $\bar{v}$ in~$\str{U}_n$ such that  
$\bar{u}\bar{v}$ is in $S^{\str{U}_n}$ and $\str{U}_n \models \psi[\bar{u}\bar{v}]$ holds.
%
\end{enumerate}

Condition (a) guarantees that any $\sigma$-alive tuple has the same 
adjacent $\sigma_i$-type  
as its original in $\fA_i$, and moreover that the originals in 
$\fA_0$ and $\fA_1$ are $\sigma$-bisimilar. This guarantees satisfaction of the 
universal requirements of $\varphi_0 \land \varphi_1$. 
Condition (b) provides witnesses for the existential~requirements~of~$\varphi_0 \land \varphi_1$. 
Considering the construction of $\str{U}$ in more detail, we describe the repair process.
Suppose $(\str{H}, \bar{h})$ is a pointed AFS, defined in the course of the induction, % 
with a $\sigma$-segment tuple $\bar{h}$, having both values 
$\bar{v}_0 \coloneqq \ori_0(\bar{h})$ and $\bar{v}_1 \coloneqq \ori_1(\bar{h})$ assigned.
The \emph{repair} of $(\str{H},\bar{h})$ is a pointed $\tau$-AFS 
$(\str{H}', \bar{h})$ constructed from~$\str{H}$ as follows:
%
\begin{enumerate}\itemsep0em
\item Let $\str{H}'$  be disjoint union of $\str{H}$ and 
isomorphic copies of $\str{A}_0^{\bar{v}_0}$ and $\str{A}_1^{\bar{v}_1}$, 
where $\str{A}_i^{\bar{v}_i}$ is the subtree of $\str{A}_i$ rooted 
at the first element of $\bar{v}_i$. We call such copies \emph{components}.

\item Identify (i.e. treat as equal) tuple $\bar{h}$ with copies of $\bar{v}_0$ and $\bar{v}_1$.
The $\tau$-adjacent type of $\bar{h}$ is then well-defined by the fact that $\bar{v}_0 \bisimto_\sigma \bar{v}_1$,
and thus we have
$\atp^{\str{H}'}_{\tau}[\bar{h}] = \textstyle \bigcup_{i=0}^{1} \atp^{\str{A}_i}_{\sigma_i}[\bar{v}_i]$.

\item For $i \in [0,1]$, define the value of $\ori_i$ to be the identity 
on all fresh copies of $\sigma_i$-alive tuples from the intersection 
of $\str{H}'$ and the copy of $\str{A}_i^{\bar{v}_i}$.
%
\end{enumerate}

\noindent Note that a repair of an AFS is simply an AFS after a routine renaming.
We can now proceed with the base case of our inductive construction~of~$\str{U}$.
Recall that $\str{U}_0$ equals $\str{A}_0 \cup \str{A}_1$, and let~$\ori_i$ 
be the identity function on $\sigma_i$-alive tuples of $\str{A}_i$.
(We take $\ori_{1{-}i}$ to be undefined for tuples from $\str{A}_i$.)
Consider the set $\mathcal{S}$ composed of all $\sigma$-segments of $\str{U}_0$,
and note that $\preceq$ is~a~well-founded order~on~$\mathcal{S}$.
Take a tuple~$\bar{u} \in \mathcal{S}$ for which all $\bar{w} \prec \bar{u}$ already 
have both $\ori_i$ defined. Let $\bar{v}_i \coloneqq \ori_i(\bar{u})$ for the 
unique $i$ for which $\ori_i(\bar{u})$ is defined, and consider the following cases:

\begin{enumerate}[label=\Roman*.]\itemsep0em
\item $\bar{u}$ shares no element with any $\bar{w} \prec \bar{u}$ from $\mathcal{S}$.
By construction, no member of $\bar{u}$ has $\ori_{1{-}i}$ defined (otherwise, there would be a tuple $\bar{w} \prec \bar{u}$ that defines $\ori_{1{-}i}$ for such an element).
As $\bar{u}$ is $\sigma$-alive we invoke $\sigma$-bisimilarity 
of $\str{A}_0$ and $\str{A}_1$ to infer the existence of
$\bar{v}_{1{-}i}$ in~$\str{A}_{1{-}i}$ 
satisfying $\bar{v}_{1{-}i} \bisimto_\sigma \bar{v}_i$.
Hence, for any adjacent map $f$ 
we can define~$\ori_{1{-}i}(\bar{u}^f) \coloneqq (\bar{v}_{1{-}i})^f$.

\item There is a tuple $\bar{w} \prec \bar{u}$ in $\mathcal{S}$ that has a common element with $\bar{u}$.
By the property $(\heartsuit)$, we know that $\bar{u}$ and any such tuple $\bar{w}$ 
can be decomposed,~respectively, as
$\bar{y}\bar{t}$ and $\bar{x}\bar{y}\bar{z}$.
Let us take $\bar{w}$ having such a $\bar{y}$ component longest.
No value of $\ori_{1{-}i}$ for a member of $\bar{t}$ is defined 
(this follows by induction, the definition of $\preceq$, 
and the fact that elements in $\mathcal{S}$~are~maximal). 
Since $\bar{w}$ is $\sigma$-alive, the inductive hypothesis 
assures us that both values 
$\bar{o}_j \coloneqq \ori_j(\bar{w}) {=} \ori_j(\bar{x}) \ori_j(\bar{y}) \ori_j(\bar{z})$  
are defined and~$\bar{o}_0 \bisimto_{\sigma} \bar{o}_1$ holds.
By invoking the last two conditions of a~bisimulation, 
we infer the existence of a $|\bar{t}|$-tuple $\bar{p}$ from $\str{A}_{1{-}i}$ 
for which $\ori_i(\bar{y})\ori_i(\bar{t})$ is $\sigma$-bisimilar 
to $\ori_{1{-}i}(\bar{y}) \bar{p}$. We put 
$\ori_{1{-}i}(\bar{u}) \coloneqq \ori_{1{-}i}(\bar{y})\bar{p}$, and 
lift it to all walks on $\bar{u}$ by setting 
$\ori_{1{-}i}(\bar{u}^f) \coloneqq \ori_{1{-}i}(\bar{u})^f$ 
for all adjacent maps $f$.
\end{enumerate}

Note that we never end  up specifying the value of the origin function for a tuple twice.
Moreover, by the choice of $\mathcal{S}$ and the fact that the values of $\ori$ for 
core tuples were lifted to all adjacent walks on them, observe that 
any~$\sigma$-alive tuple has now both values of $\ori$ defined.
Let $\str{U}_1$ be the result of performing sequentially repairs on all tuples from $\mathcal{S}$.
Observe that conditions (a) and (b) are now fulfilled.
This follows by design of repairs, relying on the any $\sigma_i$-live 
tuple $\bar{d}$ in $\str{U}_0$ is of the form $\bar{e}^f$ 
for some $\sigma$-segment $\bar{e}$ and (not necessarily surjective) adjacent map $f$.
It could be, however, that $\str{U}_1$ contains broken tuples (that by construction, 
are simply walks on $\sigma$-alive tuples).
%
Note that while constructing $\str{U}_1$ we maintained: 

\begin{center}
$(\clubsuit)${:} Let $\bar{u}$ be any $n$-fresh $\sigma$-alive tuple with either $\ori_0(\bar{u})$ or $\ori_1(\bar{u})$ undefined.\\
Then for every prefix $\bar{x}$ of $\core(\bar{u}) = \bar{x}\bar{y}$ that is contained in $\str{U}_{n{-}1}$,\\
there exists a $\sigma$-alive core tuple $\bar{t}\bar{x}\bar{z}$ that contains $\bar{x}$ as an infix.
\end{center}

The inductive step of the construction of $\str{U}_{n{+}1}$ from $\str{U}_n$ is now very similar to the base case. 
We deal with each freshly added component one by one (recall that they are~AFSs), 
defining the set $\mathcal{S}$ as before.
When assigning the origin functions however, a new case emerges. 
We may need to analyse tuples $\bar{u} \coloneqq \bar{y}\bar{t}$ in $\mathcal{S}$, where
$\bar{y}$ is $n$-aged and $\bar{t}$ is $n$-fresh, for which there is a unique 
$i$ such that $\ori_i(\bar{u})$~is~defined.
For such tuples $\bar{u}$, we define the origin functions slightly differently.
Invoke condition $(\clubsuit)$ to infer the existence of a core 
$\sigma$-alive tuple $\bar{w} \coloneqq \bar{x}\bar{y}\bar{z}$ 
with both~$\ori_0(\bar{w})$ and $\ori_1(\bar{w})$~defined, 
and $(\ori_0(\bar{x})\ \ori_0(\bar{y})\ \ori_0(\bar{z})) \bisimto_{\sigma} (\ori_1(\bar{x})\ \ori_1(\bar{y})\ \ori_1(\bar{z}))$.
From the back-and-forth conditions there exists a tuple $\bar{p}$ such that
$(\ori_i(\bar{y})\ \ori_i(\bar{t})) \bisimto_{\sigma} (\ori_{1{-}i}(\bar{y})\ \bar{p})$.
We put $\ori_{1{-}i}( (\bar{y}\bar{t})^f ) \coloneqq (\ori_{1{-}i}(\bar{y})\ \bar{p})^f$ for all adjacent maps $f$,
and then proceed as in the base case (after noting that our construction preserves $(\clubsuit)$).
This finalizes the construction~of~$\str{U}$.

By conditions (a) and (b), we infer that $\str{U}$ is the desired model of $\varphi_0$ and $\varphi_1$.
By~\cref{lemma:super-lemma-about-CIP} we can now conclude: 
\begin{theorem}
The guarded adjacent fragment has the Craig Interpolation Property.\@ 
\end{theorem}


